Reconfiguration of Distributed Information Fusion System ? A case study

Information Fusion Systems are now widely used in different fusion contexts, like scientific processing, sensor networks, video and image processing. One of the current trends in this area is to cope with distributed systems. In this context, we have defined and implemented a Dynamic Distributed Information Fusion System runtime model. It allows us to cope with dynamic execution supports while trying to maintain the functionalities of a given Dynamic Distributed Information Fusion System. The paper presents our system, the reconfiguration problems we are faced with and our solutions.

==> abstract.tex <==
%file: abstract.tex
%encoding : utf8
%description: control and verification of distributed information fusion system, dcds09
%date: 2009-04-16
%author: Olivier PASSALACQUA
%email: olivier.passalacqua@univ-savoie.fr
%LISTIC, Polytech'Savoie-Annecy, Universit\'e de Savoie
%LaTeX2e



\begin{abstract}                % Abstract of not more than 250 words.
Information Fusion Systems are now widely used in different fusion contexts,
like scientific processing, sensor networks, video and image processing.
One of the current trends in this area is to cope with distributed systems.
In this context, we have defined and implemented
a Dynamic Distributed Information Fusion System runtime model.
It allows us to cope with dynamic execution supports while trying to maintain the
functionalities of a given Dynamic Distributed Information Fusion System.
The paper presents our system, the reconfiguration problems we are faced with and our
solutions.
\end{abstract}


%end of file abstract.tex

